The implicit fairness criterion of unconstrained learning

We clarify what fairness guarantees we can and cannot expect to follow from unconstrained machine learning. Specifically, we characterize when unconstrained learning on its own implies group calibration, that is, the outcome variable is conditionally independent of group membership given the score. We show that under reasonable conditions, the deviation from satisfying group calibration is upper bounded by the excess risk of the learned score relative to the Bayes optimal score function. A lower bound confirms the optimality of our upper bound. Moreover, we prove that as the excess risk of the learned score decreases, it strongly violates separation and independence, two other standard fairness criteria. Our results show that group calibration is the fairness criterion that unconstrained learning implicitly favors. On the one hand, this means that calibration is often satisfied on its own without the need for active intervention, albeit at the cost of violating other criteria that are at odds with calibration. On the other hand, it suggests that we should be satisfied with calibration as a fairness criterion only if we are at ease with the use of unconstrained machine learning in a given application.

==> 03_03_one_side_sep.tex <==
% !TeX root = main.tex 


%\section{Results} 

\subsection{Results for separation error}
\begin{align*}
\rho^+_{f_B} &= \E_A  q_A \cdot \left|\frac{\Zbar }{\qbar} -  \frac{Z_A}{q_A} \right|  \\
&= \frac{1}{\qbar}\E_A \left|q_A \Zbar - \qbar Z_A \right|  \\
&= \frac{1}{\qbar}\E_A \left|q_A (\E_{A'}Z_{A'}) - (\E_{A'}q_{A'}) Z_A \right|  \\
\end{align*}
Next, notice that we have that for any value of $q_A$, we must have the bound $q_A^2 \le Z_A \le q_A $, which is saturated when $f_B(X,A) = q_A$ with probability $1$ for all $X$, and when $f_B = 1$ with probability $q_A$ for any $X$. 


==> 05_c_lower_bound_proof_sketch.tex <==
% !TeX root = icml_main.tex 

\subsection{Proof sketch of lower bound}\label{sec:lb_proof_sketch}



In this section, we shall sketch a proof of the lower bound~\eqref{eq:delta_lb} in Theorem~\ref{thm:main_lb}.  



 The properties of the least squares estimator are standard, and deferred to Appendix~\ref{proof:fls_performance}. 
%
Since $\fhat \in \F$, we shall write $\fhat = f_{\what}$ for some $\what \in \R^2$.
%
 We begin by given a precise characterization of the calibration error:
\begin{lemma}\label{lem:error_sphere} Let $\wst,\wA \in \calS^1$, and suppose that either $\what = 0$, or $\mathrm{span}(\what,\wA) = \R^2$. Then, for $(X,Y) \sim \Dwst$, 
\iftoggle{sigconf}
{
	\begin{align*}
	&\Delta_{f_{\what},\Dwst}(\Awa) = \frac{\sqrt{\Phi(\what;\wst)}}{2\pi},\\
	&\text{where } \Phi(\what;\wst) = \begin{cases}  1 - \langle \wst, \frac{\what}{\|\what\|}\rangle^2 & \what \ne 0 \\
	1 & \what = 0 \end{cases}~.
	\end{align*}
}
{
\begin{align*}
\Delstrong_{f_{\what},\Dwst}(\Awa) \ge \Delweak_{f_{\what},\Dwst}(\Awa) = \frac{\sqrt{\Phi(\what;\wst)}}{2\pi}, \quad \text{where}~ \Phi(\what;\wst) = \begin{cases}  1 - \langle \wst, \frac{\what}{\|\what\|}\rangle^2 & \what \ne 0 \\
1 & \what = 0 \end{cases}~.
\end{align*}
}
\end{lemma}
At the heart of Lemma~\ref{lem:error_sphere} is noting that when $\what$ and $w$ are linearly independent, then $f_{\what}(X)$ and $A_w(X) = \sign(|\langle X, w \rangle|)$ uniquely determine $X \in \sphereone$. Hence, $\E[Y|f_{\what}(X), A_w(X)] = \E[Y|X] = f_{w_*}(X)$. In the proof of Lemma~\ref{lem:error_sphere}, we show that a similar simplification occurs in the case that $\what = 0$. Because the attribute $\Awa$ is independent of the distribution $\Dwst$, and because $\wA \unifsim \sphereone$, we have that, for any $\wst$,
\begin{align}
\Pr_{\wA, S^n \sim \Dwst}[\{\mathrm{span}(\wA,\what) = \R^2\} \cup \{\what = 0\}] = 1 \label{eq:full_span},
\end{align}
so that the conditions of Lemma~\ref{lem:error_sphere} hold with probability one. 


Next, we observe that $\Phi(\what;\wst)$ corresponds to the square norm of the projection of $\wst$ onto a direction perpendicular to $\what$, or equivalently, the square of the sign of the angle between $\what$ and $\wst$. Note that calibration can occur when the angle between $\what$ and $\wst$ is either close to zero, or close to $\pi$-radians; this is in contrast to prediction, where a small loss implies that the angle between $\what$ and $\wst$ is necessarily close to zero. Nevertheless, we can still prove an information theoretic lower bound on the probability that $\Phi(\what;\wst)$ is small by a reduction to binary hypothesis testing. This is achieved in the next proposition:
\begin{proposition}\label{prop:info} For any $n \ge 1$, $\delta \in (0,1)$, and any estimator $\what$,
\iftoggle{sigconf}
{
\begin{align*}
\E_{\wst \unifsim \calS^1}\Pr_{S^n \sim \Dwst}\left[\Phi(\what;\wst) \le \min\left\{\frac{1}{2}, \frac{3\log (\sfrac{1}{\delta})}{n}\right\} \right] \le 1- \frac{\delta}{4}.
\end{align*}
}
{
	\begin{align*}
\E_{\wst \unifsim \calS^1}\Pr_{S^n \sim \Dwst}\left[\Phi(\what;\wst) \le \min\left\{\frac{1}{2}, \frac{3\log (1/\delta)}{n}\right\} \right] \le 1- \frac{\delta}{4}.
\end{align*}
}
\end{proposition}
The first part of Theorem~\ref{thm:main_lb}, Equation~\eqref{eq:delta_lb}, now follows immediately from combining the bound in Proposition~\ref{prop:info},~\eqref{eq:full_span}, and the computation of $\Delta_{f_{\what},\Dwst}(\Awa)$ in Lemma~\ref{lem:error_sphere}. The proof of Lemma~\ref{lem:error_sphere} and Proposition~\ref{prop:info} are deferred to Sections~\ref{proof:lem:error_sphere} and~\ref{proof:prop:info}, respectively. 

%

%
%\lnote{to add a picture showing the projection on the unit circle etc.}
%
%\begin{figure}[H]
%	\centering
%	\begin{tikzpicture}[scale=3]
%	\draw[step=.5cm, lightgray, very thin] (-1.2,-1.2) grid (1.2,1.2); 
%%	\filldraw[fill=green!20,draw=green!50!black] (0,0) -- (3mm,0mm) arc (0:30:3mm) -- cycle; 
%	\draw[->] (-1.25,0) -- (1.25,0) coordinate (x axis);
%	\draw[->] (0,-1.25) -- (0,1.25) coordinate (y axis);
%	\draw (0,0) circle (1cm);
%	\draw[->](30:1cm) -- (30:1cm |- x axis);
%	\draw[very thick,blue] (30:0cm |- y axis) -- node[right=2pt,fill=white] {$w_*$} (0,0);
%	\draw[very thick,blue] (30:1cm |- x axis) -- node[below=2pt,fill=white] {$\Phi(\hat{w}, w_*)$} (0,0);
%	\draw[very thick,red] (0,0) -- (30:1cm)--node[above=2pt, fill=white] {$\hat{w}$} (0,0);
%	\foreach \x/\xtext in {-1, -0.5/-\frac{1}{2}, 1} 
%	\draw (\x cm,1pt) -- (\x cm,-1pt) node[anchor=north,fill=white] {$\xtext$};
%	\foreach \y/\ytext in {-1, -0.5/-\frac{1}{2}, 0.5/\frac{1}{2}, 1} 
%	\draw (1pt,\y cm) -- (-1pt,\y cm) node[anchor=east,fill=white] {$\ytext$};
%	\end{tikzpicture}
%	\caption{Illustration of $\Phi(\hat{w}, w_*)$}
%\end{figure}


==> 11_separation.tex <==
% !TeX root = main.tex 

\section{}
Separation is 
\begin{align*}
\Delsep_f(a,y;A) :=  \left|\E_{X}[\left[\E[f \mid Y,A ] - \E[f \mid Y] \mid A = a, Y = y\right] \right| \text{ and } \Delsep_{f}(A) := \E_{a \sim A}\Delsep_f(a;A)
\end{align*}
By Jensen's inequality
\begin{align*}
|\Delsep_{f_1}(a;A) - \Delsep_{f_2}(a;A)| \le \E_{X,Y}\left[\left|\E[f_1 - f_2 \mid Y,A] - \E[f_1 - f_2 | Y]\right| \mid A = a\right]  = \Delsep_{f_1 - f_2}(a;A),
\end{align*}
which implies that $|\Delsep_{f_1}(A) - \Delsep_{f_2}(A)| \le \Delsep_{f_1 - f_2}(A)$. Moreover, we have the bound
\begin{align*}
\Delsep_f(A) &= \E_{X,Y,A}\left[|\E[f \mid Y,A ] - \E[f \mid Y]|\right] \\
&\le \E_{X,Y,A}\left[\E[|f| \mid Y,A ] + \E[|f| \mid Y]\right] \le 2\E|f|.
\end{align*}
Hence, we conclude that 
\begin{align*}
\Delsep_{f}(A)
\end{align*}



==> a4_add_results.tex <==
% !TeX root = main.tex 

\section{Additional result}

The following corollary provides a bound on the worst possible calibration error for any one group $A=a$.
\begin{corollary}[Single group calibration]\label{cor:worst_group}
	Denote the single group calibration error as\[\Delta_f^{a} = \E_{X|A=a}\left| \E[Y\mid f(X,a)] - \E[Y\mid f(X,a),A=a]\right|\] and $p_a = \Pr\{A=a\}$.
	Under Assumption \ref{asm}, we have \[ \Delta_{f}^{a} \le \frac{C'}{p_a}\sqrt{\calL(f) - \calL^*}  \]
\end{corollary}
\begin{proof}
	Note that $\sum_{a\in \calA}\Delta_f^{a}  \Pr\{A=a\} = \Delta_f(A)$. Then the desired inequality follows from Theorem \ref{thm:main_upper}.
\end{proof}
As shown in the above result, we can use our bound on a score with small calibration error $\Delta_f(A)$ to derive a bound on single group calibration error. However, the upper bound deteriorates as the mass of the single group $\Pr\{A=a\}$ decreases. In other words, Theorem \ref{thm:main_upper} implies small single group calibration error as long as the group is large enough and the excess risk of the score is small.



==> a4_examples.tex <==
% !TeX root = main.tex 
\subsection{Further Examples for Calibration and Sufficiency Bounds\label{sec:further_examples}}
We present two further examples under which one can meaningfully bound the excess risk, and consequently the sufficiency and calibration gaps, in the incomplete information setting.
In the next example, we examine sufficiency when $\fhat$ is precisely the uncalibrated Bayes score $\func$. The following lemma establishes an upper bound on the sufficiency gap of the uncalibrated Bayes score in terms of the conditional mutual information between $Y$ and $A$, conditioning on $\classx$. It is proved in Appendix~\ref{proof:lem:uncalibbayes} as a simple consequence of Tao's inequality. 
\begin{example}[Sufficiency for uncalibrated Bayes score]\label{ex:uncalibbayes} Suppose $X$ and $A$ are discrete $\calD$-measurable random variables, and $\F$ is the set of all functions $f:\X \to [0,1]$. Denote $f^* = \argmin_{f\in \F} \calL(f)$. Then, under Assumption \ref{asm}, $f^* = \E[Y\mid X]$ and  
	\[ \sufgap_{f^*}(A) \leq \sqrt{2\log2 I(Y;A \mid X)}.\]
\end{example}

Lastly, we consider an example when the attribute $\attx$ is continuous, and there exists a function $g$ which approximately predicts $A$ from $X$.
%
%function class restriction into account in our upper bound, we require additional regularity conditions. The following is an example of how one might bound the excess risk in the incomplete information setting, assuming that $\attx$ is continuous and that there exists a function $g$ which predicts $A$ from $X$ up to some accuracy. 
%
A formal statement and proof is given in Appendix~\ref{proof:ex:contA}.

\begin{example}[Sufficiency for continuous group attribute $\attx$]\label{ex:contA} Suppose there exists $g:\clspace \to\attspace$ such that $\E[|\attx - g(\classx)|] \leq \delta_1$. Let $\Ftil = \{f:\clspace \times \attspace \to [0,1] \textnormal{ s.t. } f(x,g(x)) \in \F \}$. Denote $f^* = \arg\inf_{f\in \F}L(f)$. Then, under regularity conditions, there exists constants $c_1$ and $c_2$ such that
	\[ \max\{\sufgap_{f^*}(A) ,\calgap_{f^*}(A) \} \leq c_2\sqrt{\min_{f\in \tilde{\F}}\calL(f) - \calL(\fbayes) +c\delta_1}.\]
\end{example}

The above result shows that in the incomplete information setting we may be able to bound the sufficiency gap of the population risk minimizer of class $\F$ by the approximation error for an auxiliary class $\Ftil$ up to an additional error term that accounts for how well $g(X)$ predicts $A$.
%
In other words, a score obtained by ERM will have low calibration gap with respect to any group attribute $\attx$ that is sufficiently encoded in the features that are used by the score, $\classx$, up to the flexibility allowed by the chosen class $\F$. Thus, our theoretical results also suggest that ERM can achieve simultaneous approximate sufficiency and calibration with respect to all such group attributes.


\begin{comment}

\subsection{Proof of Example~\ref{ex:uncalibbayes}}\label{proof:lem:uncalibbayes}

For $f = \E[Y\mid X]$, we have the following identity for $\Delta_f(A)$ by the tower rule: 
\begin{align*} \Delta_f(A) = \E|\E[Y\mid f] - \E[Y\mid f,A]| = \E| \E[Y\mid X] - \E[Y \mid X,A] |
\end{align*}

By applying Tao's inequality \citep{Tao2006SzemerdisRL,ahlswede07}, we have that 
\begin{align*} \E| \E[Y\mid X] - \E[Y \mid X,A] | \leq   \sqrt{2\log2 I(Y;A\mid X)} 
\end{align*}

Note that  $I(Y;(X,A)\mid X) = I(Y;A\mid X)$ and the result follows.




\subsection{Restatement and proof of Example~\ref{ex:contA}}\label{proof:ex:contA}

We first restate Example~\ref{ex:contA} more formally in the following lemma:

\begin{lemma}[Calibration and sufficiency for continuous group attribute $\attx$]
	Suppose (1) $\ell$ is the logistic loss, and (2) there exists $g:\clspace \to\attspace$ such that $\E[|\attx - g(\classx)|] \leq \delta_1$. Let $\tilde{F} = \{f:\clspace \times \attspace \to [0,1] \textnormal{ s.t. } f(x,g(x)) \in \F \}$. Denote $f^* = \arg\inf_{f\in \F}L(f)$ and $\tilde{f} = \arg\inf_{f\in \tilde{F}}L(f)$. Further suppose (3) $\tilde{f}$ is $\beta$-Lipschitz in its second argument, that is $\forall x, |\tilde{f}(x,a) -\tilde{f}(x, a')| \leq \beta|a-a'|$ and (4) $\Pr\{\delta_2 < \tilde{f} < \delta_3\} = 1$ for some $\delta_2, \delta_3 \in (0,1)$. Then, 
	\[\max\{\Delweak_{f^*}(A),\Delstrong_{f^*}(A)  \} \leq C \sqrt{\min_{f\in \tilde{\F}}\calL(f) - \calL(\fbayes) +\beta\frac{\delta_1}{\min\{\delta_2, 1-\delta_3\}}} , \]
	where $C$ is a universal constant.
\end{lemma}

\begin{proof}
	By computation, we have
		\begin{align*}
		\calL(f^*) - \calL(\fbayes) &= \E[\ell(f^*(\classx), Y)] - \calL(\fbayes)\\
		& \leq \E[\ell(\tilde{f}(\classx, g(\classx)), Y)] - \calL(\fbayes)   \\
		&\leq \E[\ell(\tilde{f}(\classx, A), Y)] - \calL(\fbayes) +\beta\frac{\delta_1}{\min\{\delta_2, 1-\delta_3\}}  \\
		&= \min_{f\in \tilde{\F}}\calL(f) - \calL(\fbayes) +\beta\frac{\delta_1}{\min\{\delta_2, 1-\delta_3\}}.
		\end{align*}
		The last inequality follows from the fact that $\forall y, ~\ell(\cdot, y)$ is $\frac{1}{\min\{\delta_2, 1-\delta_3\}}$-Lipschitz on $[\delta_2, \delta_3]$, and that $\tilde{f}$ is only supported on $[\delta_2, \delta_3]$. Then the conclusion follows from Theorem~\ref{thm:main_upper}.
\end{proof}
\end{comment}

==> old_intro.tex <==
% !TeX root = main.tex 

The scholarly debate around fairness in machine learning has happened to place much weight on a formal criterion known as \emph{group calibration}. A risk score is calibrated for a group, if the risk score obviates the need to solicit group membership for the purpose of predicting an outcome variable of interest. More formally, group membership is conditionally independent of the outcome variable given the score. A violation of group calibration therefore corresponds to the possibly undesirable scenario where the same risk score represents different outcome distributions for the group and its complement.

The concept of calibration has a venerable history in statistics and machine learning~\citep{Cox58,murphy77,dawid82,degroot83,platt99probabilisticoutputs, Zadrozny01,nicu05}. %that refers to the agreement between observed outcomes and predicted probabilities. 
The somewhat surprising appearance of calibration as a widely adopted and discussed ``fairness criterion'' largely resulted from a recent debate around fairness in recidivism prediction and pre-trial detention. After journalists at ProPublica pointed out that a popular recidivism risk score had a disparity in false positive rates between white defendants and black defendants~\cite{angwin2016machine}, the organization that produced these scores countered that this disparity was a mere consequence of the fact that their scores were calibrated by race~\cite{dieterich16compas}. Formal trade-offs dating back the 1970s confirm the observed tension between group calibration and other involved classification criteria~\cite{darlington1971another,chould16fair,kleinberg16inherent,barocas-hardt-narayanan}.

Implicit in this debate is the view that calibration is a constraint that needs to be actively enforced as a means of promoting fairness. Consequently, recent literture has proposed new learning algorithms which ensure approximate group calibration in different settings~\cite{hebert-johnson18multi,kearns2017preventing}.%, especially when there are many, intersecting protected groups. 

The goal of this work is to understand when approximate group calibration can be achieved by \emph{unconstrained} machine learning alone. By defining several relaxations of the exact calibration criterion, we show that approximate group calibration is often a routine consequence of empirical risk minimization. 

In particular, we demonstrate that many measures of mis-calibration are upper bounded by the excess risk relative to a Bayes-optimal score function. \lnote{Moritz comment: don't throw out 'excess risk' in the intro without giving context/defining it for the reader.} Provided that our model class can capture group membership given the available features, and we have sufficient data, group calibration will follow from empirical risk minimization. In fact, we don't even need to know exactly what groups (e.g. race, gender) we're concerned with ahead of time. 

We also prove lower bounds which demonstrate that, in the worst case, no other algorithm can produce score functions that are substantially better-calibrated than those found by empirical risk minimization. It is an interesting direction for future work to understand if there exists favorable conditions under which one can out-perform empirical risk minimization.


Our findings shed light on why models obtained from unconstrained machine learning are typically already well-calibrated in practice \maxs{citation?}.
Many have criticized the ways in which unconstrained machine learning can have harmful societal impact~\cite{crawford2013hidden,barocas2016big,crawford17trouble}. However, our results confirm that focusing on calibration alone cannot and will not alleviate all of these concerns. Avoiding social harm therefore requires adopting other notions of fairness criteria, scuh as modifying our notion of calibration to ensure uniformly accurate scoring across groups (see, e.g.~\cite{hebert-johnson18multi}).

%The flip side of our findings is that calibration is fairly easy to achieve and typically does not always necessitate an active intervention. In fact, we don't even need to know exactly what groups (e.g. race, gender) we're concerned with ahead of time. Provided that our model class can capture group membership given the available features, group calibration will follow from empirical risk minimization. 

Finally, we perform an extensive experimental verification of our theoretical findings on a standard machine learning dataset, demonstrating the strong connection between empirical risk and group calibration, as well as effectiveness of empirical risk minimization in achieving approximate calibration with respect to multiple group attributes simultaneously.


\lnote{Also talk about results on separation.}





